Size-Driven Quantum Phase Transitions

Can the properties of the thermodynamic limit of a many-body quantum system be extrapolated by analysing a sequence of finite-size cases? We present a model for which such an approach gives completely misleading results: a translationally invariant, local Hamiltonian on a square lattice with open boundary conditions and constant spectral gap, which has a classical product ground state for all system sizes smaller than a particular threshold size, but a ground state with topological degeneracy for all system sizes larger than this threshold. Starting from a minimal case with spins of dimension 6 and threshold lattice size 15 x 15, we show that the latter grows faster than any computable function with increasing local spin dimension. The resulting effect may be viewed as a new type of quantum phase transition that is driven by the size of the system rather than by an external field or coupling strength. We prove that the construction is thermally robust, opening the possibility that these effects are accessible to experimental observation.

==> figures/tiles.tex <==
\newcommand{\dx}{0.02}
\newcommand{\ts}{.95cm}
\newcounter{tx}
\newcounter{ty}

\usepackage{xparse}

% stripe pattern
\makeatletter
\tikzset{
    hatch distance/.store in=\hatchdistance,
    hatch distance=4pt,
    hatch thickness/.store in=\hatchthickness,
    hatch thickness=2pt
}
\pgfdeclarepatternformonly[\hatchdistance,\hatchthickness]{stripey}
    {\pgfqpoint{-1pt}{-1pt}}% below left
    {\pgfqpoint{\hatchthickness}{10pt}}% above right
    {\pgfqpoint{\hatchdistance}{10pt}}% offset to next
    {
        \pgfsetcolor{\tikz@pattern@color}
        \pgfsetlinewidth{\hatchthickness}
        \pgfpathmoveto{\pgfqpoint{0pt}{-1pt}}
        \pgfpathlineto{\pgfqpoint{0pt}{10pt}}
        \pgfusepath{stroke}
    }
\makeatother


% tiles environment
\DeclareDocumentEnvironment{tiles}{ s O{1} }{%
  \setcounter{tx}{0}%
  \setcounter{ty}{0}%
  \IfBooleanTF{#1}{%
    \begin{tikzpicture}[
      draw=black,
      font=\scriptsize,
      line width=\dx*\ts,
      x=#2*\ts,y=#2*\ts,
      baseline={([yshift=-.6ex]current bounding box.center)}
    ]
  }{%
    \begin{tikzpicture}[
    draw=black,
    font=\scriptsize,
    line width=\dx*\ts,
    x=#2*\ts,y=#2*\ts
    ]
  }%
}{
  \end{tikzpicture}%
}

\renewcommand\${
\setcounter{tx}{0}
\addtocounter{ty}{-1}
}
\newcommand{\tile}[1]{
  \addtocounter{tx}{1}
  \addtocounter{ty}{0}
  \begin{scope}[
    shift={(\thetx,\thety)}
  ]
  \node (North) at (0.5, 1) {};
  \node (South) at (0.5, 0) {};
  \node (East) at (1,0.5) {};
  \node (West) at (0,0.5) {};
  \node (Center) at (0.5,0.5) {};
  #1
  \draw (0,0) rectangle (1,1);
  \end{scope}
}

\newcommand{\arrow}[2]{
\draw[->] (#1.center) -- (#2.center);
}


% tile fillings
\DeclareDocumentCommand{\defineEdge}{ m m m m m }{
	\DeclareDocumentCommand{#1}{ m o m O{black} }{% colour, 2nd colour, text, text colour
		\IfNoValueTF{##2}{
		    \draw[fill=##1] (#2) -- (#3) -- (.5,.5) -- cycle;
	    }{
		    \draw[preaction={fill=##1}, pattern=stripey, pattern color=##2] (#2) -- (#3) -- (.5,.5) -- cycle;
		}
		\path[fill=black] (#5) circle[radius=.05];
		\node[##4] at (#4) {##3};
	}
}
\defineEdge\edgeN{0,1}{1,1}{.5,.82}{.5,1}
\defineEdge\edgeE{1,1}{1,0}{.78,.5}{1,.5}
\defineEdge\edgeS{0,0}{1,0}{.5,.18}{.5,0}
\defineEdge\edgeW{0,0}{0,1}{.22,.5}{0,.5}

\newcommand{\sidelabel}[2]{
    \node[above]  at #2 {#1};
}

% stars
\DeclareDocumentCommand{\defineStar}{m m}{
	\DeclareDocumentCommand{#1}{m O{black} m}{%
		\draw (.5,.5) -- (#2);
       % \path[fill=black] (.5,.5) circle[radius=.05];
        \path[draw=black,fill=##1] (#2) circle[radius=.275] node[##2] {##3};
	}
}
\defineStar\starN{.5,1}
\defineStar\starE{1,.5}
\defineStar\starS{.5,0}
\defineStar\starW{0,.5}

